Contracts for Interacting Two-Party Systems

This article deals with the interrelation of deontic operators in contracts -- an aspect often neglected when considering only one of the involved parties. On top of an automata-based semantics we formalise the onuses that obligations, permissions and prohibitions on one party impose on the other. Such formalisation allows for a clean notion of contract strictness and a derived notion of contract conflict that is enriched with issues arising from party interdependence.

==> eptcsdata.tex <==
\providecommand{\firstpage}{21}
\providecommand{\publicationstatus}{G. J. Pace and A. P. Ravn: \\
Proceedings of Sixth Workshop on Formal Languages\\
and Analysis of Contract-Oriented Software (FLACOS'12)\\
EPTCS 94, 2012, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.94.3}{10.4204/EPTCS.94.3}}

